Pareto Optimal Learning for Estimating Large Language Model Errors

Large Language Models (LLMs) have shown impressive abilities in many applications. When a concrete and precise answer is desired, it is important to have a quantitative estimation of the potential error rate. However, this can be challenging due to the text-in-text-out nature of generative models. We present a method based on Pareto optimization that generates a risk score to estimate the probability of error in an LLM response by integrating multiple sources of information. We prove theoretically that the error estimator optimized in our framework aligns with the LLM and the information sources in an Pareto optimal manner. Experimental results show that the risk scores estimated by our method are well correlated with the true LLM error rate, thus facilitating error correction. By dynamically combining with prompting strategies such as self-verification and information retrieval, we demonstrate the proposed method can be utilized to increase the performance of an LLM, surpassing state-of-the-art task specific models.

==> pareto.tex <==
\section{Introduction}


\section{Problem Setup}
In the most general setting, consider the joint distribution of input and output pair $(x,y) \in \mathcal{X} \times \mathcal{Y}$. In the typical supervised learning setting, the general practice is to gather samples $(x_i, y_i)$, $i=1, \cdots, n$ with enough size $n$, and fit a model $h \in \mathcal{H}: \mathcal{X} \rightarrow \mathcal{Y}$. While the input samples $x_i$'s are usually abundant, the corresponding output samples $y_i$'s usually requires manual labeling. In the weak supervision setting, we are unable to observe the ground truth label $y$ (or only a small development set). In stead, we have access to $m$ weak supervision sources, each giving a weak label $\lambda_j \in \mathcal{Y}\cup\{0\}, j =1, \cdots, m$. Each weak label does not necessarily have 100\% coverage, where 0 stands for the case of abstain, and they are not individually perfectly accurate ($\mathbb{P}(\lambda_j = y | \lambda_j \neq 0) < 1$). The problem is to still fit a predictive model $\hat{y} = h(x)$, based on observing a large enough sample with weak labels: $(x_i, \lambda_i)$, $i=1, \cdots, n$. In this section, we restrict to binary classification for simplicity, where $y \in \mathcal{Y} = \{-1, 1\}$. 


\subsection{Label model}\label{sec-label_model}
In almost all of of the previous work, there is a label model, either explicitly or implicitly, to aggregate the output from different sources $\lambda_1, \cdots, \lambda_m$ into: 1. a single hard label $\tilde{y} \in \{-1, 1\}$, 2. a probabilistic soft label $\mathbb{P}(\tilde{y} = 1 | \lambda_1, \cdots, \lambda_m)$. In either case, let's denote the label model as a function
\[
\psi(\lambda_1, \cdots, \lambda_m): \{-1, 0, 1\}^m \rightarrow \left\lbrace\begin{array}{cl} 
   \{-1, 1\} & \mbox{hard label} \\
   \left[0, 1 \right]  & \mbox{soft label}
\end{array} \right.
\]

After the weak labels are aggregated into a single output, an end model $h \in \mathcal{H}: \mathcal{X} \rightarrow \mathcal{Y}$ is trained on the weakly labeled dataset, taking the label model output $\psi(\lambda_1, \cdots, \lambda_m): \{-1, 1\}$ as the target. Precisely, the learning goal is to minimize the generalization loss:
\begin{equation}\label{eq-fit_end}
    \min_{h \in \mathcal{H}} \quad \mathbb{E} [\ell(h(x), \psi(\lambda_1, \cdots, \lambda_m))].
\end{equation}


However, there is no guarantee that solving problem \ref{eq-fit_end} leads to a predictive model for the true label $y$, if there is no assumption that the weak labels $\lambda_1, \cdots, \lambda_m$ are consistent with $y$ at some level. In many of the previous literature, various assumptions are imposed on the weak label distribution, e.g. independence, better-than-random-guess accuracy, etc. The fundamental belief is that the weak sources each ``helps in the right direction" in finding the ground truth. In this section, we encode this belief not by putting assumptions on the weak sources, but regulating the behavior of the label model in the most general way, summarized into the following definition. \\

\begin{definition}[Consistent label model]\label{def:consistent_lm}
A label model $\psi(\lambda_1, \cdots, \lambda_m)$ is defined as being \textit{consistent}, if for $\forall \vec{\lambda}, \vec{\lambda}' \in \{-1, 0, 1\}^m$, it satisfies
\begin{align}
    \lambda_j \geq \lambda_j', \ \forall j=1, \cdots, m \quad \rightarrow \quad \psi(\lambda_1, \cdots, \lambda_m) \geq \psi(\lambda_1', \cdots, \lambda_m'). 
\end{align}
\end{definition}

In other words, if some sources possibly switch towards positive (negative), with all the other sources staying the same, a reasonable label model should not switch towards negative (positive). The same definition applies to both hard label and soft label cases. 


\subsection{Multi-objective learning}\label{sec-multi}
In this section we are going to introduce a different approach for self-supervision, namely multi-objective learning. In stead of fitting an end model to the aggregated label as in Equation \ref{eq-fit_end}, we consider the following multi-objective optimization problem

\begin{equation}\label{eq-fit_end}
    \min_{h \in \mathcal{H}} \quad \mathbb{E} [\ell_1(h(x), \lambda_1)], \cdots, \mathbb{E} [\ell_m(h(x), \lambda_m))].
\end{equation}

where a single model $h(x)$ is trained to minimize the loss on \textit{all} supervision sources simultaneously. This problem, however, is ill-posed, as the sources may conflict, and there does not exist a solution that optimized every objective function. To address the issue, we use the concept of Pareto efficiency, and resort to finding a Pareto optimal solution $h^*$, such that there does not exist $h' \in \mathcal{H}$, s.t. for $\forall x \in \mathcal{X}$, we have
\[
\mathbb{E} [\ell_j(h'(x), \lambda_j)] \leq \mathbb{E} [\ell_j(h^*(x), \lambda_j))], \ \forall j=1, \cdots, m, 
\]
and for some $1 \leq k \leq m$, there is strict advantage
\[
\mathbb{E} [\ell_k(h'(x), \lambda_k)] < \mathbb{E} [\ell_k(h^*(x), \lambda_k))].
\]

However, even with the definition of Pareto efficiency, there usually exist multiple Pareto optimal solutions. Overtime researchers have developed many approaches to find or approximate the Pareto optimal solutions. One typical and most suitable approach for multi-objective learning is through scalarization using a multivariate function \cite{hwang2012multiple}. To align with the Pareto efficiency definition, we define the following multi-objective loss function. \\

\begin{definition}[Pareto loss function]\label{def:pareto_loss}
A Pareto loss function is any function $\zeta: \mathbb{R}^m \rightarrow \mathbb{R}$ that satisfies 
\begin{align}
    \zeta(u_1, \cdots, u_m) \leq \zeta(v_1, \cdots, v_m)
\end{align}
if 
\begin{align}
    u_j \geq v_j, \ \forall j=1, \cdots, m,
\end{align}
where the each entry is the margin variable
\[
u_j = \lambda_j \cdot h(x).
\]
\end{definition}

In the ordinary single objective learning case where $m=1$, we can easily verify that the loss functions we are familiar with, such as the logistic loss, hinge loss, 0/1 loss, etc., all satisfies the Pareto loss definition. Therefore, minimizing the Pareto loss in the multi-objective learning scenario is a generalization to the typical machine learning practice. 


\subsection{Equivalence of the two approaches}

In this section we are going to show that the typical label model approach in Section \ref{sec-label_model}, is mathematically equivalent to multi-objective learning through minimizing some Pareto loss function, as described in Section \ref{sec-multi}. Specifically, we state the following theorems establishing the mathematical equivalence.

\begin{theorem}[Hard-label equivalence]\label{theorem-hard_eq}
For any hard-label label model $\psi: \{-1, 0, 1\}^m \rightarrow \{-1, 1\}$ that is consistent as defined in Def. \ref{def:consistent_lm}, we can always find some Pareto loss function $\zeta: \mathbb{R}^m \rightarrow \mathbb{R}$ as defined in Def. \ref{def:pareto_loss}, s.t. the problem
\begin{align}
    \min_{h \in \mathcal{H}} \quad \mathbb{E}[ \zeta(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x))]
\end{align}
has an optimal solution of $h(x) \equiv \psi(\vec{\lambda}(x))$.

\end{theorem}

\begin{proof}
See appendix.
\end{proof}

Theorem \ref{theorem-hard_eq} states that for any possible label model that is consistent with the sources, the model always arise in the optimal solution of minimizing some Pareto loss function. Therefore, instead of constructing a label model, we can alternatively design a Pareto loss function on the multiple sources to get an end model. To generalize the equivalence to the soft-label scenario, we need the following requirement.

\begin{definition}[Symmetric label model]\label{def:symmetric_lm}
A soft-label label model $\psi: \{-1, 0, 1\}^m \rightarrow [0,1]$ is defined as being \textit{symmetric} if
\begin{align}
    \psi(-\lambda_1, \cdots, -\lambda_m) = 1 - \psi(\lambda_1, \cdots, \lambda_m).
\end{align}
A soft-label label model $\psi: \{-1, 0, 1\}^m \rightarrow [0,1]$ is defined as being \textit{weakly symmetric}, if there exist an odd function $\phi: \{-1, 0, 1\}^m \rightarrow \mathbb{R}$, an class balance offset constant $a \in \mathbb{R}$, and an uni-variate function $\psi_0: \mathbb{R} \rightarrow [0,1]$ satisfying $\psi_0(-u) = 1 - \psi_0(u)$, s.t.
\[
\psi(\lambda_1, \cdots, \lambda_m) = \psi_0(\phi(\lambda_1, \cdots, \lambda_m) + a).
\]
\end{definition}

In other words, if all supervision sources change sign, the estimated soft-label probability should switch to the opposite value as well (up to class balance adjustment in the weak case). Many of the label models in the previous literature, including soft-label majority vote, factor graph model, Ising model, etc., all satisfy this condition. \\

\begin{theorem}[Soft-label equivalence]\label{theorem-soft_eq}
For any soft-label label model $\psi: \{-1, 0, 1\}^m \rightarrow [0, 1]$ that is consistent as defined in Def. \ref{def:consistent_lm} and (weakly) symmetric as defined in Def. \ref{def:symmetric_lm}, we can always find a Pareto loss function $\zeta: \mathbb{R}^m \rightarrow \mathbb{R}$ as defined in Def. \ref{def:pareto_loss}, s.t. the problem
\begin{align}
    \min_{h \in \mathcal{H}} \quad \mathbb{E} [\zeta(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x))]
\end{align}
is optimized when $h(x)$ is randomized with $\mathbb{P}(h(x) = 1) \equiv \psi(\vec{\lambda}(x))$.

\end{theorem}

\begin{proof}
    See appendix.
\end{proof}




\appendix
\section{Proof of Theorems}

\begin{theorem}[Hard-label equivalence]\label{theorem-hard_eq}
For any hard-label label model $\psi: \{-1, 0, 1\}^m \rightarrow \{-1, 1\}$ that is consistent as defined in Def. \ref{def:consistent_lm}, we can always find some Pareto loss function $\zeta: \mathbb{R}^m \rightarrow \mathbb{R}$ as defined in Def. \ref{def:pareto_loss}, s.t. the problem
\begin{align}
    \min_{h \in \mathcal{H}} \quad \mathbb{E}[ \zeta(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x))]
\end{align}
has an optimal solution of $h(x) \equiv \psi(\vec{\lambda}(x))$.

\end{theorem}

\begin{proof}
We prove by constructing such Pareto loss function. Notice that the definition of consistent label model and the the definition of Pareto loss function have similar format, let's construct our loss function as
\[
\zeta(u_1, \cdots, u_m) = \psi(-u_1, \cdots, -u_m) - \psi(u_1, \cdots, u_m).
\]
One can easily verify that $\zeta: \{-1, 0, 1\}^m \rightarrow \{-2, -1, 0, 1, 2\}$ is a Pareto loss function. The problem now becomes
\begin{align}
    \min_{h \in \mathcal{H}} \quad & \mathbb{E}[ \psi(-\lambda_1 \cdot h(x), \cdots, -\lambda_m \cdot h(x)) - \psi(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x))] \\
    &= \sum_{x \in \mathcal{X}} p(x) \cdot \left(\psi(-\lambda_1 \cdot h(x), \cdots, -\lambda_m \cdot h(x)) - \psi(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x))\right) \\
    &= \sum_{x \in \mathcal{X}} p(x) \cdot (\psi(-\vec{\lambda}(x) \cdot h(x)) - \psi(\vec{\lambda}(x) \cdot h(x)))
\end{align}
Now consider each individual $x \in \mathcal{X}$. Let $h(x)$ be the class prediction for $x$ s.t. $h(x) = \pm 1$. Let's discuss the optimal strategy to choose $h(x)$ in the following cases.
\begin{itemize}
    \item[Case 1:] $\psi(\vec{\lambda}(x)) = 1, \psi(-\vec{\lambda}(x)) = -1$. 
    In this case, choosing $h(x) = 1 = \psi(\vec{\lambda}(x))$ gives 
    \[
    \psi(-\vec{\lambda}(x)) - \psi(\vec{\lambda}(x)) = -2
    \]
    which is the lowest possible value.

    \item[Case 2:] $\psi(\vec{\lambda}(x)) = -1, \psi(-\vec{\lambda}(x)) = 1$. 
    In this case, choosing $h(x) = -1 = \psi(\vec{\lambda}(x))$ gives 
    \[
    \psi(\vec{\lambda}(x)) - \psi(-\vec{\lambda}(x)) = -2
    \]
    which is the lowest possible value.

    \item[Case 3:] $\psi(\vec{\lambda}(x)) = \psi(-\vec{\lambda}(x))$. 
    In this case, choosing any $h(x)$, we will have the same value
    \[
    \pm ( \psi(-\vec{\lambda}(x)) - \psi(\vec{\lambda}(x))) = 0.
    \]
\end{itemize}

Therefore, for $\forall x \in \mathcal{X}$, $h(x) = \psi(\vec{\lambda}(x))$ is always the optimal solution. 
\end{proof}



\begin{theorem}[Soft-label equivalence]\label{theorem-soft_eq}
For any soft-label label model $\psi: \{-1, 0, 1\}^m \rightarrow [0, 1]$ that is consistent as defined in Def. \ref{def:consistent_lm} and (weakly) symmetric as defined in Def. \ref{def:symmetric_lm}, we can always find a Pareto loss function $\zeta: \mathbb{R}^m \rightarrow \mathbb{R}$ as defined in Def. \ref{def:pareto_loss}, s.t. the problem
\begin{align}
    \min_{h \in \mathcal{H}} \quad \mathbb{E} [\zeta(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x))]
\end{align}
is optimized when $h(x)$ is randomized with $\mathbb{P}(h(x) = 1) \equiv \psi(\vec{\lambda}(x))$.

\end{theorem}

\begin{proof}
    We prove by constructing such Pareto loss function. Let the loss function be
\[
\zeta(u_1, \cdots, u_m) = -\log(\psi(u_1, \cdots, u_m))
\]

The problem now becomes
\begin{align}
    \min_{h \in \mathcal{H}} \quad & \mathbb{E}[ -\log (\psi(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x)))] \\
    &= \mathbb{E}_x \mathbb{E}_h[ -\log (\psi(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x)))] \\
    &= \sum_{x \in \mathcal{X}} p(x) \cdot \mathbb{E}_h[ -\log (\psi(\lambda_1 \cdot h(x), \cdots, \lambda_m \cdot h(x)))] \\
    &= \sum_{x \in \mathcal{X}} p(x) \cdot (-p_h(x)\log(\psi(\vec{\lambda}(x))) - (1-p_h(x))\log(\psi(-\vec{\lambda}(x))),
\end{align}
where $p_h(x)$ is the predicted positive class probability of $h(x)$. Let's consider each individual $x \in \mathcal{X}$and discuss the following two cases based on the symmetric property of $\psi$.

\begin{itemize}
    \item[Case 1:] $\psi$ is symmetric. Now the problem is to minimize
    \[
    \ell(p_h(x)) = -p_h(x)\log(\psi(\vec{\lambda}(x))) - (1-p_h(x))\log(1 - \psi(\vec{\lambda}(x))
    \]
    Taking derivative w.r.t. $p_h(x)$, we have
    \[
    \ell'(p_h(x)) = -p_h(x)\log(\psi(\vec{\lambda}(x))) - (1-p_h(x))\log(1 - \psi(\vec{\lambda}(x))
    \]
\end{itemize}
\end{proof}


